Towards Realistic Few-Shot Relation Extraction: A New Meta Dataset and Evaluation

We introduce a meta dataset for few-shot relation extraction, which includes two datasets derived from existing supervised relation extraction datasets NYT29 (Takanobu et al., 2019; Nayak and Ng, 2020) and WIKIDATA (Sorokin and Gurevych, 2017) as well as a few-shot form of the TACRED dataset (Sabo et al., 2021). Importantly, all these few-shot datasets were generated under realistic assumptions such as: the test relations are different from any relations a model might have seen before, limited training data, and a preponderance of candidate relation mentions that do not correspond to any of the relations of interest. Using this large resource, we conduct a comprehensive evaluation of six recent few-shot relation extraction methods, and observe that no method comes out as a clear winner. Further, the overall performance on this task is low, indicating substantial need for future research. We release all versions of the data, i.e., both supervised and few-shot, for future research.

==> table/statisticsDataBackup.tex <==
\begin{comment}
*************************************************************paper
*************************************************************
**********Fewshot TACRED Statistics**************************
------------------------------
Relation Distribution for TACRED train: 
{'no_relation': 59961, 'per:title': 2443, 'per:employee_of': 1524, 'org:alternate_names': 808, 'per:countries_of_residence': 445, 'org:city_of_headquarters': 382, 'per:cities_of_residence': 374, 'org:subsidiaries': 296, 'per:spo
use': 258, 'org:stateorprovince_of_headquarters': 229, 'per:other_family': 179, 'org:members': 170, 'per:parents': 152, 'per:date_of_death': 134, 'per:cause_of_death': 117, 'org:website': 111, 'org:political/religious_affiliatio
n': 105, 'org:shareholders': 76, 'org:number_of_employees/members': 75, 'per:charges': 72, 'per:city_of_birth': 65, 'per:religion': 53, 'per:stateorprovince_of_birth': 38, 'per:country_of_birth': 28, 'org:dissolved': 23, 'per:co
untry_of_death': 6}
Pos Tag Distribution for train: 
Entity Pos Tags:
{'NNP': 91691, 'PRP': 10240, 'NN': 10126, 'PRP$': 8208, 'CD': 7457, 'JJ': 2640, 'NNPS': 2224, 'NNS': 1914, 'RB': 941, 'RBR': 92, 'VB': 91, 'VBG': 80, 'VBN': 78, 'POS': 70, 'DT': 62, 'IN': 54, 'FW': 46, 'TO': 46, 'LS': 40, 'VBP':
 30, 'VBZ': 25, '``': 25, 'CC': 15, 'VBD': 14, 'UH': 10, 'SYM': 10, 'MD': 6, 'JJS': 4, 'WP': 3, 'JJR': 2, ':': 1, "''": 1, '$': 1, 'WDT': 1}
NNP 67.2971346368387 %
PRP 7.515706652574717 %
NN 7.4320356996066 %
PRP$ 6.024308613704421 %
CD 5.473107862133756 %
JJ 1.9376431213669192 %
NNPS 1.6323175386060713 %
NNS 1.4047912629910164 %
RB 0.6906523398508602 %
RBR 0.06752392695672597 %
VB 0.06678997122893547 %
VBG 0.058716458223239974 %
VBN 0.057248546767658975 %
POS 0.05137690094533498 %
DT 0.04550525512301098 %
IN 0.03963360930068698 %
FW 0.03376196347836299 %
TO 0.03376196347836299 %
LS 0.029358229111619987 %
VBP 0.02201867183371499 %
VBZ 0.018348893194762492 %
`` 0.018348893194762492 %
CC 0.011009335916857495 %
VBD 0.010275380189066995 %
UH 0.007339557277904997 %
SYM 0.007339557277904997 %
MD 0.004403734366742998 %
JJS 0.0029358229111619985 %
WP 0.002201867183371499 %
JJR 0.0014679114555809993 %
: 0.0007339557277904996 %
'' 0.0007339557277904996 %
$ 0.0007339557277904996 %
WDT 0.0007339557277904996 %
Traversing:  test
------------------------------
Relation Distribution for TACRED test: 
{'no_relation': 14705, 'org:top_members/employees': 346, 'per:origin': 132, 'per:stateorprovinces_of_residence': 81, 'org:founded_by': 68, 'per:siblings': 55, 'per:children': 37, 'per:schools_attended': 30, 'per:city_of_death': 
28, 'org:member_of': 18, 'per:date_of_birth': 9}
Pos Tag Distribution for test: 
Entity Pos Tags:
{'NNP': 18471, 'PRP': 3638, 'PRP\$': 3005, 'NN': 2538, 'CD': 1555, 'JJ': 700, 'NNS': 373, 'NNPS': 228, 'RB': 194, 'VBG': 174, 'RBR': 21, 'VB': 19, 'FW': 19, 'DT': 14, 'POS': 11, 'VBN': 9, '``': 9, 'VBD': 6, 'TO': 5, 'IN': 5, 'UH'
: 5, 'VBP': 4, 'JJS': 4, 'CC': 4, 'LS': 1, 'VBZ': 1, ',': 1, 'MD': 1, 'WP': 1, "''": 1, ':': 1}
NNP 59.549293958346766 %
PRP 11.728673673350958 %
PRP$ 9.687923141401766 %
NN 8.18234573473467 %
CD 5.0132181314075694 %
RBR 0.06770262428267458 %
JJ 2.256754142755819 %
NNS 1.2025275646398865 %
NNPS 0.7350570636404669 %
RB 0.625443290992327 %
VBG 0.5609646011993036 %
RBR 0.06770262428267458 %
VB 0.06125475530337224 %
FW 0.06125475530337224 %
DT 0.04513508285511639 %
POS 0.03546327938616287 %
VBN 0.029015410406860533 %
`` 0.029015410406860533 %
VBD 0.019343606937907022 %
TO 0.01611967244825585 %
IN 0.01611967244825585 %
UH 0.01611967244825585 %
VBP 0.012895737958604681 %
JJS 0.012895737958604681 %
CC 0.012895737958604681 %
LS 0.0032239344896511702 %
VBZ 0.0032239344896511702 %
, 0.0032239344896511702 %
MD 0.0032239344896511702 %
WP 0.0032239344896511702 %
'' 0.0032239344896511702 %
: 0.0032239344896511702 %
Traversing:  dev

------------------------------
Relation Distribution for TACRED dev: 
{'no_relation': 21998, 'per:age': 243, 'org:country_of_headquarters': 177, 'org:parents': 96, 'per:stateorprovince_of_death': 41, 'org:founded': 38, 'per:alternate_names': 38}
Pos Tag Distribution for dev: 
Entity Pos Tags:
{'NNP': 28172, 'PRP': 4122, 'NN': 3630, 'PRP\$': 3464, 'CD': 2563, 'NNPS': 1059, 'JJ': 1041, 'NNS': 637, 'RB': 274, 'FW': 41, 'POS': 35, 'RBR': 33, 'DT': 27, 'VB': 25, 'VBG': 24, 'TO': 23, 'VBP': 17, '``': 16, 'IN': 16, 'VBN': 11, 'CC': 9, 'VBD': 7, 'WP': 4, 'VBZ': 3, 'SYM': 3, 'LS': 2, 'UH': 2, 'JJR': 1, 'MD': 1}
NNP 62.24205735495559 %
PRP 9.106977155229552 %
NN 8.019972603950334 %
PRP$ 7.6532190358358 %
CD 5.662586717334629 %
NNPS 2.3397110158631964 %
JJ 2.299942556670054 %
NNS 1.4073615836684195 %
RB 0.6053643232733861 %
FW 0.09058371260660156 %
POS 0.07732755954222084 %
RBR 0.07290884185409394 %
DT 0.05965268878971323 %
VB 0.05523397110158632 %
VBG 0.05302461225752287 %
TO 0.05081525341345942 %
VBP 0.037559100349078695 %
`` 0.03534974150501524 %
IN 0.03534974150501524 %
VBN 0.024302947284697982 %
CC 0.019884229596571074 %
VBD 0.01546551190844417 %
WP 0.00883743537625381 %
VBZ 0.006628076532190359 %
SYM 0.006628076532190359 %
LS 0.004418717688126905 %
UH 0.004418717688126905 %
JJR 0.0022093588440634526 %
MD 0.0022093588440634526 %


************************************************************
*************************************************************
******* Fewshoot NYT Statistics************
************************************************************
------------------------------
Relation Distribution for NYT train: 
{'/location/location/contains': 26517, 'no_relation': 22265, '/people/person/nationality': 8090, '/people/person/place_lived': 6865, '/location/country/capital': 6680, '/business/person/company': 5338, '/business/company/founder
s': 783, '/location/us_state/capital': 631, '/people/ethnicity/geographic_distribution': 507, '/business/company/place_founded': 461, '/people/person/children': 460, '/people/person/ethnicity': 135, '/location/us_county/county_s
eat': 93, '/people/deceased_person/place_of_burial': 23, '/people/place_of_interment/interred_here': 23, '/film/film_location/featured_in_films': 14}
Pos Tag Distribution for train: 
Entity Pos Tags:
{'NNP': 154583, 'NN': 1579, 'JJ': 712, 'NNPS': 439, 'NNS': 340, 'VB': 24, 'RB': 20, 'VBZ': 17, 'VBD': 16, 'VBG': 15, 'VBP': 12, 'VBN': 7, 'UH': 3, 'JJR': 1, 'PRP\$': 1, 'FW': 1}
NNP 97.97997084363314 %
NN 1.0008239842809152 %
JJ 0.4512898523166635 %
NNPS 0.27825315332445966 %
NNS 0.21550358116245166 %
VB 0.015212017493820118 %
RB 0.012676681244850099 %
VBZ 0.010775179058122584 %
VBD 0.010141344995880078 %
VBG 0.009507510933637574 %
VBP 0.007606008746910059 %
VBN 0.004436838435697535 %
UH 0.0019015021867275148 %
JJR 0.0006338340622425049 %
PRP$ 0.0006338340622425049 %
FW 0.0006338340622425049 %
Traversing:  test
------------------------------
Relation Distribution for NYT test: 
{'no_relation': 6728, '/location/country/administrative_divisions': 631, '/location/administrative_division/country': 631, '/location/neighborhood/neighborhood_of': 549, '/people/deceased_person/place_of_death': 191, '/business/
company/major_shareholders': 29}
Pos Tag Distribution for test: 
Entity Pos Tags:
{'NNP': 17186, 'NN': 165, 'JJ': 79, 'NNS': 45, 'NNPS': 38, 'VBZ': 2, 'VB': 2, 'RB': 1}
NNP 98.10480648475854 %
NN 0.9418883434181984 %
JJ 0.45096472200022836 %
NNS 0.2568786391140541 %
NNPS 0.21691973969631237 %
VBZ 0.011416828405069072 %
VB 0.011416828405069072 %
RB 0.005708414202534536 %
Traversing:  dev
------------------------------
Relation Distribution NYT for dev: 
{'no_relation': 5669, '/people/person/place_of_birth': 146, '/location/province/capital': 11, '/sports/sports_team/location': 10, '/business/company_advisor/companies_advised': 8, '/business/company/advisors': 8, '/people/person
/religion': 5, '/film/film/featured_film_locations': 2}
Pos Tag Distribution for dev: 
Entity Pos Tags:
{'NNP': 11466, 'JJ': 125, 'NN': 78, 'NNPS': 21, 'NNS': 11, 'VBZ': 3, 'IN': 3, ',': 3, 'VBN': 3, 'RB': 2, 'VB': 1, 'PRP\$': 1, '-LRB-': 1}
NNP 97.84946236559139 %
JJ 1.0667349377026796 %
NN 0.6656426011264721 %
NNPS 0.17921146953405018 %
NNS 0.0938726745178358 %
VBZ 0.025601638504864313 %
IN 0.025601638504864313 %
, 0.025601638504864313 %
VBN 0.025601638504864313 %
RB 0.017067759003242873 %
VB 0.008533879501621437 %
PRP$ 0.008533879501621437 %
-LRB- 0.008533879501621437 %



**************************************************
**************************************************
********** Fewshot WikiData Statistics************
------------------------------
Relation Distribution for Wikidata train: 
{'no_relation': 503978, 'located in the administrative territorial entity': 63773, 'shares border with': 37290, 'sport': 36011, 'country of citizenship': 21391, 'part of': 15077, 'league': 10301, 'occupation': 9363, 'diplomatic 
relation': 6854, 'continent': 5478, 'contains administrative territorial entities': 5432, 'position held': 5281, 'member of': 4841, 'author': 4820, 'headquarters location': 3769, 'date of death': 3236, 'spouse': 2664, 'sister ci
ty': 2600, 'characters': 1731, 'location': 1558, 'date of birth': 1556, 'educated at': 1495, 'located on terrain feature': 1327, 'notable work': 1187, 'instrument': 1083, 'award received': 1066, 'record label': 1046, 'owned by':
 1044, 'located on astronomical body': 1029, 'named after': 1019, 'screenwriter': 928, 'publisher': 917, 'languages spoken or written': 753, 'manufacturer': 738, 'original language of work': 735, 'successful candidate': 594, 'fi
eld of this occupation': 555, 'licensed to broadcast to': 529, 'work location': 521, 'main subject': 512, 'opposite of': 511, 'production company': 463, 'noble family': 444, 'sister': 382, 'family name': 382, 'parent astronomica
l body': 366, 'constellation': 359, 'facet of': 307, 'sports discipline competed in': 303, 'separated from': 292, 'material used': 270, 'replaces': 251, 'organisation directed from the office': 250, 'heritage status': 241, 'moth
er': 227, 'librettist': 219, 'basin country': 213, 'voice type': 210, 'discoverer or inventor': 200, 'adjacent station': 198, 'location of formation': 191, 'candidate': 189, 'architect': 186, 'use': 177, 'nominated for': 176, 'f
irst performance': 167, 'territory claimed by': 166, 'language of work or name': 155, 'crosses': 154, 'operating system': 152, 'designer': 133, 'studies': 129, 'terminus': 126, 'writing system': 120, 'ethnic group': 114, 'filmin
g location': 114, 'head of government': 107, 'official residence': 98, 'measured physical quantity': 98, 'military rank': 95, 'doctoral advisor': 86, 'highest point': 83, 'head coach': 79, 'religious order': 78, 'office held by 
head of government': 75, 'cause of death': 73, 'relative': 72, 'native language': 71, 'diocese': 67, 'officeholder': 67, 'astronaut mission': 60, 'noble title': 59, 'manner of death': 59, 'time of spacecraft launch': 55, 'execut
ive producer': 54, 'located on street': 53, 'date of official opening': 50, 'period': 47, 'currency': 47, 'edition or translation of': 46, 'website account on': 44, 'maintained by': 43, 'business division': 41, 'signatory': 38, 
'lake outflow': 38, 'sidekick of': 37, 'primary destinations': 36, 'chief executive officer': 36, 'stock exchange': 36, 'illustrator': 36, 'deity of': 35, 'connecting service': 35, 'operating area': 34, 'tracklist': 34, 'basic f
orm of government': 32, 'afflicts': 31, 'terminus location': 30, 'software engine': 27, 'medical specialty': 26, 'highway system': 26, 'public holiday': 25, 'place of detention': 24, 'vessel class': 23, 'patron saint': 23, 'voic
e actor': 22, 'endemic to': 22, 'history of topic': 21, 'contains settlement': 20, 'significant drug interaction': 20, 'inspired by': 19, 'numeric value': 19, 'has immediate cause': 19, 'symptoms': 18, 'parent club': 18, 'time o
f spacecraft landing': 18, 'lakes on river': 17, 'spin-off': 17, 'home world': 17, 'has dialect': 17, 'film editor': 16, 'commissioned by': 16, 'anthem': 15, 'interaction': 15, 'anatomical location': 15, 'substitute/deputy/repla
cement of office/officeholder': 14, 'underlies': 14, 'origin of the watercourse': 13, 'fictional analog of': 13, 'academic degree': 13, 'used by': 12, 'executive body': 12, 'medical condition': 11, 'color': 11, 'wing configurati
on': 11, 'ortholog': 11, 'readable file format': 10, 'choreographer': 10, 'cathedral': 10, 'tonality': 10, 'central bank/issuer': 10, 'target': 10, 'lake inflows': 10, 'exclave of': 10, 'has parts of the class': 10, 'patron': 9,
 'CPU': 9, 'sexual orientation': 9, 'main regulatory text': 9, 'distribution': 9, 'instruction set': 9, 'coat of arms': 9, 'standards body': 9, 'location of discovery': 9, 'temporal range start': 8, 'approved by': 8, 'legislated
 by': 8, 'cell component': 8, 'flag': 7, 'translator': 7, 'space launch vehicle': 7, 'chromosome': 7, 'venous drainage': 6, 'list of works': 6, 'parent(s) of this hybrid': 6, 'located in time zone': 6, 'mascot': 6, 'source of en
ergy': 6, 'GUI toolkit or framework': 6, 'commemorates': 5, 'powerplant': 4, 'dedicated to': 4, 'input set': 4, 'mushroom ecological type': 4, 'dual to': 4, 'catalog': 3, 'codomain': 3, 'has contributing factor': 3, 'office held
 by head of state': 3, 'genetic association': 3, 'taxon synonym': 3, 'taxonomic type': 3, 'service retirement': 2, 'product certification': 2, 'encodes': 2, 'coincident with': 2, 'notation': 2, 'exemplar of': 1, 'time of earlies
t written record': 1, 'mother house': 1, 'companion of': 1, 'Human Development Index': 1, 'depends on software': 1}
Pos Tag Distribution for train: 
Entity Pos Tags:
{'NNP': 1173799, 'NN': 208082, 'CD': 61742, 'JJ': 50379, 'NNPS': 24664, 'NNS': 19941, 'RB': 2592, 'VBN': 1840, 'VBG': 1787, 'PRP\$': 1432, 'PRP': 1269, 'VB': 1183, 'VBP': 889, 'VBD': 539, 'VBZ': 506, 'DT': 333, 'IN': 295, 'TO': 2
00, 'WP': 66, 'UH': 55, 'WRB': 41, 'JJR': 33, 'PDT': 22, 'JJS': 21, 'EX': 19, 'FW': 17, 'CC': 16, '.': 15, 'MD': 15, 'WDT': 10, 'RBR': 9, 'RBS': 8, 'RP': 7, ',': 6, '-RRB-': 3, ':': 1, '``': 1, '-LRB-': 1}
NNP 75.63927420259074 %
NN 13.408744984979101 %
CD 3.9786369453512545 %
JJ 3.2464084524286685 %
NNPS 1.5893411554556596 %
NNS 1.284992376781597 %
RB 0.1670277438753272 %
VBN 0.11856907744236189 %
VBG 0.11515377249429386 %
PRP$ 0.09227767331383817 %
PRP 0.08177399960562894 %
VB 0.07623218402951855 %
VBP 0.05728690752514116 %
VBD 0.03473300692469188 %
VBZ 0.03260649629664952 %
DT 0.021458425428427453 %
IN 0.019009716220378673 %
TO 0.012887943200256729 %
WP 0.00425302125608472 %
UH 0.0035441843800706 %
WRB 0.002642028356052629 %
JJR 0.00212651062804236 %
PDT 0.00141767375202824 %
JJS 0.0013532340360269564 %
EX 0.001224354604024389 %
FW 0.001095475172021822 %
CC 0.0010310354560205382 %
. 0.0009665957400192546 %
MD 0.0009665957400192546 %
WDT 0.0006443971600128364 %
RBR 0.0005799574440115528 %
RBS 0.0005155177280102691 %
RP 0.0004510780120089855 %
, 0.0003866382960077018 %
-RRB- 0.0001933191480038509 %
: 6.443971600128364e-05 %
`` 6.443971600128364e-05 %
-LRB- 6.443971600128364e-05 %
Traversing:  test

------------------------------
Relation Distribution for Wikidata test: 
{'no_relation': 513112, 'country': 81394, 'instance of': 38796, 'subclass of': 14126, 'cast member': 10114, 'publication date': 10044, 'place of birth': 9304, 'genre': 8339, 'capital': 7662, 'country of origin': 5047, 'member of political party': 4743, 'original network': 4065, 'position played on team / speciality': 3759, 'director': 3729, 'mouth of the watercourse': 2506, 'brother': 1798, 'composer': 1580, 'official language': 1554, 'employer': 1438, 'creator': 1355, 'located next to body of water': 1200, 'founder': 1102, 'item operated': 1028, 'father': 1007, 'military branch': 1003, 'based on': 731, 'producer': 659, 'influenced by': 639, 'occupant': 521, 'has quality': 481, 'movement': 478, 'field of work': 461, 'connecting line': 451, 'winner': 378, 'student': 365, 'given name': 361, 'said to be the same as': 334, 'is a list of': 266, 'drafted by': 256, 'product': 244, 'lyrics by': 205, 'enclave within': 193, 'depicts': 187, 'from fictional universe': 183, 'country for sport': 156, 'political ideology': 151, 'head of state': 119, 'has cause': 118, 'conferred by': 114, 'programming language': 110, 'office contested': 109, 'architectural style': 97, 'presenter': 94, 'airline alliance': 88, 'airline hub': 86, 'surface played on': 80, 'organizer': 74, 'foundational text': 71, 'canonization status': 71, 'list of episodes': 59, 'IUCN conservation status': 50, 'instrumentation': 49, 'killed by': 48, 'convicted of': 47, 'license': 42, 'place of publication': 40, 'editor': 35, 'minor planet group': 35, 'culture': 34, 'director of photography': 29, 'radio format': 26, 'antiparticle': 24, 'affiliation': 22, 'contributor': 13, 'describes the fictional universe': 13, 'professional or sports partner': 12, 'carries': 12, 'geography of topic': 11, 'arterial supply': 10, 'highest judicial authority': 9, 'track gauge': 7, 'sex or gender': 6, 'manifestation of': 6, 'Solid solution series with': 6, 'ancestral home': 5, 'Fach': 5, 'fabrication method': 5, 'points/goal scored by': 4, 'electoral district': 3, 'published in': 3, 'location of landing': 1, 'home port': 1}
Pos Tag Distribution for test: 
Entity Pos Tags:
{'NNP': 1110554, 'NN': 197141, 'CD': 59903, 'JJ': 48461, 'NNS': 28040, 'NNPS': 19748, 'RB': 3890, 'VBN': 1991, 'VBG': 1805, 'PRP\$': 1775, 'PRP': 1342, 'VB': 1187, 'VBP': 818, 'VBD': 529, 'VBZ': 399, 'DT': 364, 'IN': 287, 'TO': 157, 'WP': 93, 'JJS': 52, 'WRB': 48, 'FW': 47, 'JJR': 42, 'MD': 31, 'UH': 31, 'EX': 13, 'RBR': 12, '.': 11, 'CC': 10, ',': 7, 'PDT': 7, '-RRB-': 4, 'RP': 4, '-LRB-': 3, 'RBS': 3, 'POS': 3, 'WP\$': 2, '``': 1, 'WDT': 1}
NNP 75.09751044078506 %
NN 13.331002639949798 %
CD 4.050740592473979 %
JJ 3.277013502694047 %
NNS 1.89611148378162 %
NNPS 1.3353926384350723 %
RB 0.263048276459005 %
VBN 0.13463473481487892 %
VBG 0.12205710514357432 %
PRP$ 0.12002845519658971 %
PRP 0.09074827429511176 %
VB 0.08026691623569125 %
VBP 0.05531452188778049 %
VBD 0.035771860731828704 %
VBZ 0.026981044294895375 %
DT 0.024614286023413326 %
IN 0.019407417826152813 %
TO 0.010616601389219483 %
WP 0.006288814835652305 %
JJS 0.003516326574773332 %
WRB 0.0032458399151753838 %
FW 0.0031782182502758964 %
JJR 0.002840109925778461 %
MD 0.002096271611884102 %
UH 0.002096271611884102 %
EX 0.000879081643693333 %
RBR 0.0008114599787938459 %
. 0.0007438383138943588 %
CC 0.0006762166489948716 %
, 0.0004733516542964101 %
PDT 0.0004733516542964101 %
-RRB- 0.00027048665959794865 %
RP 0.00027048665959794865 %
-LRB- 0.00020286499469846148 %
RBS 0.00020286499469846148 %
POS 0.00020286499469846148 %
WP$ 0.00013524332979897432 %
`` 6.762166489948716e-05 %
WDT 6.762166489948716e-05 %
Traversing:  dev

------------------------------
Relation Distribution for Wikidata dev: 
{'no_relation': 236148, 'member of sports team': 3414, 'performer': 3197, 'follows': 2161, 'inception': 1878, 'place of death': 1191, 'participant of': 755, 'conflict': 592, 'developer': 345, 'platform': 312, 'series': 266, 'applies to jurisdiction': 263, 'subsidiary': 190, 'industry': 122, 'child': 113, 'religion': 102, 'narrative location': 95, 'deepest point': 93, 'different from': 62, 'partner': 60, 'legislative body': 47, 'distributor': 44, 'residence': 42, 'home venue': 38, 'place of burial': 37, 'significant event': 34, 'time of discovery': 31, 'allegiance': 30, 'appointed by': 29, 'has facet polytope': 17, 'natural product of taxon': 17, 'place served by airport': 11, 'collection': 10, 'represents organisation': 10, 'service entry': 8, 'driving side': 5, 'found in taxon': 5, 'represented by': 4, 'indigenous to': 4, 'soundtrack album': 4, 'type of orbit': 3, 'species kept': 3, 'archives at': 2, 'pet': 2, 'language regulatory body': 1, 'floruit': 1, 'cause of destruction': 1, 'foods traditionally associated': 1, 'given name version for other gender': 1, 'location of final assembly': 1}
Pos Tag Distribution for dev: 
Entity Pos Tags:
{'NNP': 378240, 'NN': 72388, 'CD': 18667, 'JJ': 15642, 'NNS': 7263, 'NNPS': 6956, 'RB': 891, 'VBG': 640, 'VBN': 604, 'PRP\$': 459, 'PRP': 426, 'VB': 388, 'VBP': 295, 'VBD': 192, 'VBZ': 153, 'DT': 105, 'IN': 98, 'TO': 88, 'WP': 20, 'WRB': 13, 'UH': 12, 'JJR': 10, 'FW': 9, 'RBR': 8, 'EX': 7, 'JJS': 7, 'RP': 4, 'MD': 3, ',': 3, 'PDT': 3, '-RRB-': 2, 'SYM': 2, '.': 2, 'WDT': 1, 'RBS': 1, 'CC': 1, '-LRB-': 1}
NNP 75.10663140086258 %
NN 14.373992263762798 %
CD 3.706682234454055 %
JJ 3.1060118664665093 %
NNS 1.4422045893201803 %
NNPS 1.38124399329632 %
RB 0.17692472657087713 %
VBG 0.12708397868166257 %
VBN 0.11993550488081905 %
PRP$ 0.09114304096075487 %
PRP 0.08459027330998166 %
VB 0.07704466207575794 %
VBP 0.058577771423578846 %
VBD 0.03812519360449877 %
VBZ 0.03038101365358496 %
DT 0.020849715252460266 %
IN 0.01945973423562958 %
TO 0.017474047068728606 %
WP 0.003971374333801955 %
WRB 0.0025813933169712712 %
UH 0.0023828246002811733 %
JJR 0.0019856871669009777 %
FW 0.00178711845021088 %
RBR 0.0015885497335207822 %
EX 0.0013899810168306844 %
JJS 0.0013899810168306844 %
RP 0.0007942748667603911 %
MD 0.0005957061500702933 %
, 0.0005957061500702933 %
PDT 0.0005957061500702933 %
-RRB- 0.00039713743338019554 %
SYM 0.00039713743338019554 %
. 0.00039713743338019554 %
WDT 0.00019856871669009777 %
RBS 0.00019856871669009777 %
CC 0.00019856871669009777 %
-LRB- 0.00019856871669009777 %

\end{comment}
